On the (In)Tractability of Reinforcement Learning for LTL Objectives

In recent years, researchers have made significant progress in devising reinforcement-learning algorithms for optimizing linear temporal logic (LTL) objectives and LTL-like objectives. Despite these advancements, there are fundamental limitations to how well this problem can be solved. Previous studies have alluded to this fact but have not examined it in depth. In this paper, we address the tractability of reinforcement learning for general LTL objectives from a theoretical perspective. We formalize the problem under the probably approximately correct learning in Markov decision processes (PAC-MDP) framework, a standard framework for measuring sample complexity in reinforcement learning. In this formalization, we prove that the optimal policy for any LTL formula is PAC-MDP-learnable if and only if the formula is in the most limited class in the LTL hierarchy, consisting of formulas that are decidable within a finite horizon. Practically, our result implies that it is impossible for a reinforcement-learning algorithm to obtain a PAC-MDP guarantee on the performance of its learned policy after finitely many interactions with an unconstrained environment for LTL objectives that are not decidable within a finite horizon.

==> ijcai22-aux.tex <==
\begin{filecontents}
{ijcai22.aux}
\relax 
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyperFirstAtBeginDocument{\AtBeginDocument}
\HyperFirstAtBeginDocument{\ifx\hyper@anchor\@undefined
\global\let\oldcontentsline\contentsline
\gdef\contentsline#1#2#3#4{\oldcontentsline{#1}{#2}{#3}}
\global\let\oldnewlabel\newlabel
\gdef\newlabel#1#2{\newlabelxx{#1}#2}
\gdef\newlabelxx#1#2#3#4#5#6{\oldnewlabel{#1}{{#2}{#3}}}
\AtEndDocument{\ifx\hyper@anchor\@undefined
\let\contentsline\oldcontentsline
\let\newlabel\oldnewlabel
\fi}
\fi}
\global\let\hyper@last\relax 
\gdef\HyperFirstAtBeginDocument#1{#1}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\citation{sutton98}
\citation{pacmodelfreerl}
\citation{Dewey2014ReinforcementLA}
\citation{gltl17}
\citation{ltlprograms}
\citation{gltl17}
\citation{ufukpacmdpltl}
\citation{dorsa}
\citation{truncatedltl-rl}
\citation{omegaregularrl19}
\citation{hasanbeig2019reinforcement}
\citation{bozkurt2020control}
\citation{osbert}
\citation{rewardmachine1}
\citation{ltlrewardshaping}
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{1}{section.1}\protected@file@percent }
\newlabel{sec:introduction}{{1}{1}{Introduction}{section.1}{}}
\newlabel{sec:introduction@cref}{{[section][1][]1}{[1][1][]1}}
\@writefile{toc}{\contentsline {paragraph}{Specifying an Objective}{1}{section*.1}\protected@file@percent }
\@writefile{toc}{\contentsline {paragraph}{The Reward Objective}{1}{section*.2}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {1.1}The Linear Temporal Logic Objective}{1}{subsection.1.1}\protected@file@percent }
\citation{smcbltl}
\citation{pacmdpsmcconfidenceinterval}
\citation{ltlrewardshaping}
\citation{gltl17}
\citation{Kearns2002NearOptimalRL}
\citation{alur2021framework}
\citation{pacmodelfreerl}
\citation{smcbltl}
\citation{pacmdpsmcconfidenceinterval}
\citation{ufukpacmdpltl}
\citation{smcpmin}
\citation{dorsa}
\citation{omegaregularrl19}
\citation{hasanbeig2019reinforcement}
\citation{bozkurt2020control}
\citation{gltl17}
\citation{truncatedltl-rl}
\citation{ltlf-rl}
\citation{rewardmachine1}
\citation{Fiechter94efficientreinforcement}
\citation{Kearns2002NearOptimalRL}
\citation{kakade03}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.2}Trouble with Infinite Horizons}{2}{subsection.1.2}\protected@file@percent }
\@writefile{toc}{\contentsline {paragraph}{Our Results}{2}{section*.3}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {1.3}Implications for Relevant and Future Work}{2}{subsection.1.3}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {1.4}Contributions}{2}{subsection.1.4}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {2}Preliminaries: Reinforcement Learning}{2}{section.2}\protected@file@percent }
\newlabel{sec:preliminaries}{{2}{2}{Preliminaries: Reinforcement Learning}{section.2}{}}
\newlabel{sec:preliminaries@cref}{{[section][2][]2}{[1][2][]2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.1}Markov Processes}{2}{subsection.2.1}\protected@file@percent }
\newlabel{sec:background_markov_processes}{{2.1}{2}{Markov Processes}{subsection.2.1}{}}
\newlabel{sec:background_markov_processes@cref}{{[subsection][1][2]2.1}{[1][2][]2}}
\citation{puterman94}
\citation{approximateplanninginpompdps}
\citation{Grill2016BlazingTT}
\citation{Fiechter94efficientreinforcement}
\citation{Fiechter94efficientreinforcement}
\citation{Kearns2002NearOptimalRL}
\citation{kakade03}
\citation{valiantpaclearnable}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.2}Objective}{3}{subsection.2.2}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {2.3}Planning with a Generative Model}{3}{subsection.2.3}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {2.4}Reinforcement Learning}{3}{subsection.2.4}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {2.5}Probably Approximately Correct in MDPs}{3}{subsection.2.5}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap \MakeUppercase  {d}efinition\nobreakspace  {}1\else \numberline {1}\MakeUppercase  {d}efinition\fi }{3}{definition.1}\protected@file@percent }
\newlabel{def:rl-obj-pac-algo}{{1}{3}{}{definition.1}{}}
\newlabel{def:rl-obj-pac-algo@cref}{{[definition][1][]1}{[1][3][]3}}
\newlabel{eq:pac-obj-epsilon-delta-inequality}{{1}{3}{}{equation.2.1}{}}
\newlabel{eq:pac-obj-epsilon-delta-inequality@cref}{{[equation][1][]1}{[1][3][]3}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap \MakeUppercase  {d}efinition\nobreakspace  {}2\else \numberline {2}\MakeUppercase  {d}efinition\fi }{3}{definition.2}\protected@file@percent }
\newlabel{def:rl-obj-sample-efficiently-pac-algo}{{2}{3}{}{definition.2}{}}
\newlabel{def:rl-obj-sample-efficiently-pac-algo@cref}{{[definition][2][]2}{[1][3][]3}}
\@writefile{toc}{\contentsline {section}{\numberline {3}Linear Temporal Logic Objectives}{3}{section.3}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {3.1}Linear Temporal Logic}{3}{subsection.3.1}\protected@file@percent }
\newlabel{sec:background_ltl}{{3.1}{3}{Linear Temporal Logic}{subsection.3.1}{}}
\newlabel{sec:background_ltl@cref}{{[subsection][1][3]3.1}{[1][3][]3}}
\newlabel{eq:ltl_grammar}{{2}{3}{Linear Temporal Logic}{equation.3.2}{}}
\newlabel{eq:ltl_grammar@cref}{{[equation][2][]2}{[1][3][]3}}
\citation{tlhierarchy}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces The hierarchy of LTL\relax }}{4}{figure.caption.4}\protected@file@percent }
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{fig:ltl-hierarchy}{{1}{4}{The hierarchy of LTL\relax }{figure.caption.4}{}}
\newlabel{fig:ltl-hierarchy@cref}{{[figure][1][]1}{[1][4][]4}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.2}MDP with LTL Objectives}{4}{subsection.3.2}\protected@file@percent }
\newlabel{sec:ltl-objectives}{{3.2}{4}{MDP with LTL Objectives}{subsection.3.2}{}}
\newlabel{sec:ltl-objectives@cref}{{[subsection][2][3]3.2}{[1][4][]4}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.3}Infinite Horizons in LTL Objectives}{4}{subsection.3.3}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces Two MDPs parameterized by $p$ in range $0 < p < 1$. Action $a_1$ in the MDP on the left and action $a_2$ in the MDP on the right have probability $p$ of transitioning to the state $h$. Conversely, action $a_2$ in the MDP on the left and action $a_1$ in the MDP on the right have probability $p$ of transitioning to the state $q$. Both actions in both MDPs have probability $1 - p$ to loop around the state $g$. \relax }}{4}{figure.caption.5}\protected@file@percent }
\newlabel{fig:counterexample-mdp-simple}{{2}{4}{Two MDPs parameterized by $p$ in range $0 < p < 1$. Action $a_1$ in the MDP on the left and action $a_2$ in the MDP on the right have probability $p$ of transitioning to the state $h$. Conversely, action $a_2$ in the MDP on the left and action $a_1$ in the MDP on the right have probability $p$ of transitioning to the state $q$. Both actions in both MDPs have probability $1 - p$ to loop around the state $g$. \relax }{figure.caption.5}{}}
\newlabel{fig:counterexample-mdp-simple@cref}{{[figure][2][]2}{[1][4][]4}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.4}Intuition of the Problem}{4}{subsection.3.4}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {4}Learnability of LTL Objectives}{4}{section.4}\protected@file@percent }
\newlabel{sec:maintheoremstatement}{{4}{4}{Learnability of LTL Objectives}{section.4}{}}
\newlabel{sec:maintheoremstatement@cref}{{[section][4][]4}{[1][4][]4}}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces Counterexample MDPs $\mathcal  {M}_1$ and $\mathcal  {M}_2$, with transitions distinguished by arrow types (see legend). Both MDPs are parameterized by the parameter $p$ that is in range $0 < p < 1$. Unlabeled edges are deterministic (actions $a_1$ and $a_2$ transition with probability $1$). Ellipsis indicates a deterministic chain of states. \relax }}{5}{figure.caption.6}\protected@file@percent }
\newlabel{fig:counterexample-mdps}{{3}{5}{Counterexample MDPs $\mathcal {M}_1$ and $\mathcal {M}_2$, with transitions distinguished by arrow types (see legend). Both MDPs are parameterized by the parameter $p$ that is in range $0 < p < 1$. Unlabeled edges are deterministic (actions $a_1$ and $a_2$ transition with probability $1$). Ellipsis indicates a deterministic chain of states. \relax }{figure.caption.6}{}}
\newlabel{fig:counterexample-mdps@cref}{{[figure][3][]3}{[1][4][]5}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap \MakeUppercase  {d}efinition\nobreakspace  {}3\else \numberline {3}\MakeUppercase  {d}efinition\fi }{5}{definition.3}\protected@file@percent }
\newlabel{def:rl-ltl-pac-algo}{{3}{5}{}{definition.3}{}}
\newlabel{def:rl-ltl-pac-algo@cref}{{[definition][3][]3}{[1][4][]5}}
\newlabel{eq:pac-ltl-epsilon-delta-inequality}{{3}{5}{}{equation.4.3}{}}
\newlabel{eq:pac-ltl-epsilon-delta-inequality@cref}{{[equation][3][]3}{[1][5][]5}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap \MakeUppercase  {d}efinition\nobreakspace  {}4\else \numberline {4}\MakeUppercase  {d}efinition\fi }{5}{definition.4}\protected@file@percent }
\newlabel{def:rl-ltl-sample-efficiently-pac-algo}{{4}{5}{}{definition.4}{}}
\newlabel{def:rl-ltl-sample-efficiently-pac-algo@cref}{{[definition][4][]4}{[1][5][]5}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap \MakeUppercase  {d}efinition\nobreakspace  {}5\else \numberline {5}\MakeUppercase  {d}efinition\fi }{5}{definition.5}\protected@file@percent }
\newlabel{def:rl-ltl-pac-learnable}{{5}{5}{}{definition.5}{}}
\newlabel{def:rl-ltl-pac-learnable@cref}{{[definition][5][]5}{[1][5][]5}}
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap \MakeUppercase  {t}heorem\nobreakspace  {}1\else \numberline {1}\MakeUppercase  {t}heorem\fi }{5}{theorem.1}\protected@file@percent }
\newlabel{thm:ltl-non-pac}{{1}{5}{}{theorem.1}{}}
\newlabel{thm:ltl-non-pac@cref}{{[theorem][1][]1}{[1][5][]5}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.1}Proof of \Cref  {thm:ltl-non-pac}: Forward Direction}{5}{subsection.4.1}\protected@file@percent }
\newlabel{sec:ltlnonpacforwardproof}{{4.1}{5}{Proof of \Cref {thm:ltl-non-pac}: Forward Direction}{subsection.4.1}{}}
\newlabel{sec:ltlnonpacforwardproof@cref}{{[subsection][1][4]4.1}{[1][5][]5}}
\@writefile{toc}{\contentsline {subsubsection}{MDP Family}{5}{section*.7}\protected@file@percent }
\newlabel{sec:counterexample-mdps}{{4.1}{5}{MDP Family}{section*.7}{}}
\newlabel{sec:counterexample-mdps@cref}{{[subsection][1][4]4.1}{[1][5][]5}}
\@writefile{toc}{\contentsline {subsubsection}{Sample Complexity of $\ensuremath  {\mathsf  {F}\,}h_0$}{5}{section*.8}\protected@file@percent }
\newlabel{sec:samplecomplexityFh0}{{4.1}{5}{Sample Complexity of \texorpdfstring {$\eventually h_0$}{F h0}}{section*.8}{}}
\newlabel{sec:samplecomplexityFh0@cref}{{[subsection][1][4]4.1}{[1][5][]5}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap \MakeUppercase  {l}emma\nobreakspace  {}2\else \numberline {2}\MakeUppercase  {l}emma\fi }{5}{lemma.2}\protected@file@percent }
\newlabel{thm:minofm1m2pacprob}{{2}{5}{}{lemma.2}{}}
\newlabel{thm:minofm1m2pacprob@cref}{{[lemma][2][]2}{[1][5][]5}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap \MakeUppercase  {l}emma\nobreakspace  {}3\else \numberline {3}\MakeUppercase  {l}emma\fi }{6}{lemma.3}\protected@file@percent }
\newlabel{thm:ltlpaclowerboundFh0}{{3}{6}{}{lemma.3}{}}
\newlabel{thm:ltlpaclowerboundFh0@cref}{{[lemma][3][]3}{[1][6][]6}}
\@writefile{toc}{\contentsline {subsubsection}{Sample Complexity of Non-\ltlclasst {finitary} Formulas}{6}{section*.9}\protected@file@percent }
\newlabel{sec:samplecomplexitynonfinitary}{{4.1}{6}{Sample Complexity of \texorpdfstring {Non-\ltlclasst {finitary}}{Non-finitary} Formulas}{section*.9}{}}
\newlabel{sec:samplecomplexitynonfinitary@cref}{{[subsection][1][4]4.1}{[1][6][]6}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap \MakeUppercase  {d}efinition\nobreakspace  {}6\else \numberline {6}\MakeUppercase  {d}efinition\fi }{6}{definition.6}\protected@file@percent }
\newlabel{def:uncommittable-word}{{6}{6}{}{definition.6}{}}
\newlabel{def:uncommittable-word@cref}{{[definition][6][]6}{[1][6][]6}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap \MakeUppercase  {l}emma\nobreakspace  {}4\else \numberline {4}\MakeUppercase  {l}emma\fi }{6}{lemma.4}\protected@file@percent }
\newlabel{thm:uncommitablewordssamesatprob}{{4}{6}{}{lemma.4}{}}
\newlabel{thm:uncommitablewordssamesatprob@cref}{{[lemma][4][]4}{[1][6][]6}}
\newlabel{eq:guaranteemdplabelfunc}{{4}{6}{Sample Complexity of \texorpdfstring {Non-\ltlclasst {finitary}}{Non-finitary} Formulas}{equation.4.4}{}}
\newlabel{eq:guaranteemdplabelfunc@cref}{{[equation][4][]4}{[1][6][]6}}
\newlabel{eq:safetymdplabelfunc}{{5}{6}{Sample Complexity of \texorpdfstring {Non-\ltlclasst {finitary}}{Non-finitary} Formulas}{equation.4.5}{}}
\newlabel{eq:safetymdplabelfunc@cref}{{[equation][5][]5}{[1][6][]6}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap \MakeUppercase  {l}emma\nobreakspace  {}5\else \numberline {5}\MakeUppercase  {l}emma\fi }{6}{lemma.5}\protected@file@percent }
\newlabel{thm:ltlpaclowerbound}{{5}{6}{}{lemma.5}{}}
\newlabel{thm:ltlpaclowerbound@cref}{{[lemma][5][]5}{[1][6][]6}}
\@writefile{toc}{\contentsline {subsubsection}{Conclusion}{6}{section*.10}\protected@file@percent }
\citation{ltlf-rl}
\citation{rewardmachine1}
\citation{ipoc19}
\citation{dorsa}
\citation{omegaregularrl19}
\citation{hasanbeig2019reinforcement}
\citation{bozkurt2020control}
\citation{dorsa}
\citation{omegaregularrl19}
\citation{bozkurt2020control}
\citation{dorsa}
\citation{bozkurt2020control}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2}Proof Sketch of \Cref  {thm:ltl-non-pac}: Reverse Direction}{7}{subsection.4.2}\protected@file@percent }
\newlabel{sec:ltlnonpacreverseproofoutline}{{4.2}{7}{Proof Sketch of \Cref {thm:ltl-non-pac}: Reverse Direction}{subsection.4.2}{}}
\newlabel{sec:ltlnonpacreverseproofoutline@cref}{{[subsection][2][4]4.2}{[1][7][]7}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.3}Consequence of the Core Theorem}{7}{subsection.4.3}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {5}Empirical Justifications}{7}{section.5}\protected@file@percent }
\newlabel{sec:empirical}{{5}{7}{Empirical Justifications}{section.5}{}}
\newlabel{sec:empirical@cref}{{[section][5][]5}{[1][7][]7}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.1}Methodology}{7}{subsection.5.1}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces Left: LTL-PAC probabilities vs.\ number of samples, varying parameters $p$. Right: number of samples needed to reach 0.9 LTL-PAC probability vs.\ parameter $p$.\relax }}{7}{figure.caption.11}\protected@file@percent }
\newlabel{fig:bozkurt_pac_probs_plot}{{4}{7}{Left: LTL-PAC probabilities vs.\ number of samples, varying parameters $p$. Right: number of samples needed to reach 0.9 LTL-PAC probability vs.\ parameter $p$.\relax }{figure.caption.11}{}}
\newlabel{fig:bozkurt_pac_probs_plot@cref}{{[figure][4][]4}{[1][7][]7}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.2}Results}{7}{subsection.5.2}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {5.3}Conclusion}{7}{subsection.5.3}\protected@file@percent }
\citation{collisionavoidance2010}
\citation{rlroboticssurvey}
\citation{safeautonomousvehciles18}
\citation{smcbltl}
\citation{osbert}
\citation{pacmdpsmcconfidenceinterval}
\citation{ufukpacmdpltl}
\citation{smcpmin}
\citation{dorsa}
\citation{omegaregularrl19}
\citation{hasanbeig2019reinforcement}
\citation{bozkurt2020control}
\citation{omegaregularrl19}
\citation{bozkurt2020control}
\citation{pacmodelfreerl}
\citation{gltl17}
\citation{truncatedltl-rl}
\citation{ltlf-rl}
\citation{rewardmachine1}
\citation{rewardmachine1}
\citation{gltl17}
\bibstyle{named}
\bibdata{paper}
\bibcite{alur2021framework}{\citeauthoryear {Alur \bgroup \em  et al.\egroup }{2021}}
\@writefile{toc}{\contentsline {section}{\numberline {6}Directions Forward}{8}{section.6}\protected@file@percent }
\newlabel{sec:directions_forward}{{6}{8}{Directions Forward}{section.6}{}}
\newlabel{sec:directions_forward@cref}{{[section][6][]6}{[1][8][]8}}
\@writefile{toc}{\contentsline {subsection}{\numberline {6.1}Use a \ltlclasst {Finitary} Objective}{8}{subsection.6.1}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {6.2}Best-effort Guarantee}{8}{subsection.6.2}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {6.3}Know More About the Environment}{8}{subsection.6.3}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {6.4}Use an LTL-like Objective}{8}{subsection.6.4}\protected@file@percent }
\@writefile{toc}{\contentsline {subsubsection}{LTL-in-the-limit Objectives}{8}{section*.12}\protected@file@percent }
\@writefile{toc}{\contentsline {subsubsection}{General LTL-like Objectives}{8}{section*.13}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {7}Conclusion}{8}{section.7}\protected@file@percent }
\newlabel{sec:conclusion}{{7}{8}{Conclusion}{section.7}{}}
\newlabel{sec:conclusion@cref}{{[section][7][]7}{[1][8][]8}}
\bibcite{pacmdpsmcconfidenceinterval}{\citeauthoryear {Ashok \bgroup \em  et al.\egroup }{2019}}
\bibcite{bozkurt2020control}{\citeauthoryear {Bozkurt \bgroup \em  et al.\egroup }{2020}}
\bibcite{smcpmin}{\citeauthoryear {Br{\'a}zdil \bgroup \em  et al.\egroup }{2014}}
\bibcite{rewardmachine1}{\citeauthoryear {Camacho \bgroup \em  et al.\egroup }{2019}}
\bibcite{ipoc19}{\citeauthoryear {Dann \bgroup \em  et al.\egroup }{2019}}
\bibcite{Dewey2014ReinforcementLA}{\citeauthoryear {Dewey}{2014}}
\bibcite{Fiechter94efficientreinforcement}{\citeauthoryear {Fiechter}{1994}}
\bibcite{ufukpacmdpltl}{\citeauthoryear {Fu and Topcu}{2014}}
\bibcite{ltlf-rl}{\citeauthoryear {Giacomo \bgroup \em  et al.\egroup }{2019}}
\bibcite{Grill2016BlazingTT}{\citeauthoryear {Grill \bgroup \em  et al.\egroup }{2016}}
\bibcite{omegaregularrl19}{\citeauthoryear {Hahn \bgroup \em  et al.\egroup }{2019}}
\bibcite{hasanbeig2019reinforcement}{\citeauthoryear {Hasanbeig \bgroup \em  et al.\egroup }{2019}}
\bibcite{smcbltl}{\citeauthoryear {Henriques \bgroup \em  et al.\egroup }{2012}}
\bibcite{ltlrewardshaping}{\citeauthoryear {Jiang \bgroup \em  et al.\egroup }{2020}}
\bibcite{osbert}{\citeauthoryear {Jothimurugan \bgroup \em  et al.\egroup }{2019}}
\bibcite{kakade03}{\citeauthoryear {Kakade}{2003}}
\bibcite{Kearns2002NearOptimalRL}{\citeauthoryear {Kearns and Singh}{2002}}
\bibcite{approximateplanninginpompdps}{\citeauthoryear {Kearns \bgroup \em  et al.\egroup }{1999}}
\bibcite{rlroboticssurvey}{\citeauthoryear {Kober \bgroup \em  et al.\egroup }{2013}}
\bibcite{truncatedltl-rl}{\citeauthoryear {Li \bgroup \em  et al.\egroup }{2017}}
\bibcite{gltl17}{\citeauthoryear {Littman \bgroup \em  et al.\egroup }{2017}}
\bibcite{tlhierarchy}{\citeauthoryear {Manna and Pnueli}{1987}}
\bibcite{ltlprograms}{\citeauthoryear {Pnueli}{1977}}
\bibcite{puterman94}{\citeauthoryear {Puterman}{1994}}
\bibcite{dorsa}{\citeauthoryear {Sadigh \bgroup \em  et al.\egroup }{2014}}
\bibcite{safeautonomousvehciles18}{\citeauthoryear {Schwarting \bgroup \em  et al.\egroup }{2018}}
\bibcite{pacmodelfreerl}{\citeauthoryear {Strehl \bgroup \em  et al.\egroup }{2006}}
\bibcite{sutton98}{\citeauthoryear {Sutton and Barto}{1998}}
\bibcite{collisionavoidance2010}{\citeauthoryear {Temizer \bgroup \em  et al.\egroup }{2010}}
\bibcite{valiantpaclearnable}{\citeauthoryear {Valiant}{1984}}
\gdef \@abspage@last{9}
\end{filecontents}
